RYDE: A Digital Signature Scheme based on Rank-Syndrome-Decoding Problem with MPCitH Paradigm

We present a signature scheme based on the Syndrome-Decoding problem in rank metric. It is a construction from multi-party computation (MPC), using a MPC protocol which is a slight improvement of the linearized-polynomial protocol used in [Fen22], allowing to obtain a zero-knowledge proof thanks to the MPCitH paradigm. We design two different zero-knowledge proofs exploiting this paradigm: the first, which reaches the lower communication costs, relies on additive secret sharings and uses the hypercube technique [AMGH+22]; and the second relies on low-threshold linear secret sharings as proposed in [FR22]. These proofs of knowledge are transformed into signature schemes thanks to the Fiat-Shamir heuristic [FS86].

==> algebraic-Rank-SD.tex <==
% comparer minrank RSD

\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
\newcommand{\any}{*} % any entry of matrix, typically for submatrices
\newcommand{\minor}[2]{\left\vert #1 \right\vert_{#2}}

\newcommand{\trsp}[1]{{#1}^{\top}}

% comments
\newcommand{\mb}[1]{\textcolor{blue}{\bf Magali: #1}}
%\mb{J'essaie de ne pas me tromper sur les notations qui sont différentes de d'habitude... dans  $\bm{H}\bm{x}=\bm{y}$ les $\bm{x}$ et $\bm{y}$ sont des vecteurs colonnes, mais lignes dans Definition 1...  }



Algebraic attacks amount to solve the system of equations $\bm{H}\bm{x}=\bm{y}$
using computer algebra techniques like Gröbner basis. Today, the best
algebraic modelings for solving the Rank-SD problem are the MaxMinors
modeling~\cite{BBBGNRT20,BBCGPSTV20} and the Support Minors
modeling~\cite{BBCGPSTV20,BBBGT22}. They can both benefits from a
classical improvement that is the hybrid approach, that consists in specializing some variables with all possible values and solving the resulting system with less variables, but the same number of equations. In certain cases, the gain in complexity for solving the specialized system compared to the original one superseeds the lost in complexity coming from the exhausive search.
\paragraph{Hybrid methods}
As shown in~\cite[Section 5]{BBBGT22}, solving a Rank-SD problem of
parameters $(q,m,n,k,r)$ amount to solve $q^{ar}$ smaller Rank-SD
problems of parameters $(q,m,n-a,k-a,r)$.


\paragraph{MaxMinors Modeling}
Let $\bm{H}, \bm{x}, \bm{y}$ be a Rank-SD problem with parameters
$(q,m,n,k,r)$, i.e. $\bm{H}=(\bm{I} \; \bm{H}')\in\Fqm^{(n-k)\times n}$ is
uniformly sampled, $\bm{x}\in \Fqm^n$ has rank  exactly\footnote{We assume the rank $r$ is known. Otherwise, we can try to solve for $r=1$, $r=2$, \dots until we find the good $r$.} $r$, and
$\bm{y} = \bm{H} \bm{x}$.

The idea of the MaxMinors modeling from ~\cite{BBBGNRT20} is the following: let $\bm{E}=(E_1,\dots,E_r)$ be a basis of $\supp(\bm{x})$, and $\bm{X}=(x_{i,j})\in\Fq^{r\times n}$ a matrix representing the coordinates of $\bm{x}$ in the basis $\bm{E}$, then $\trsp{\bm{x}} = (E_1,\dots,E_r)\bm{X}$. Considering the extended code $C'$ described in the previous section, and a parity-check $\bm{H}'\in\Fqm^{(n-k-1)\times n}$ of this code, we have the relation :

\begin{align*}
\bm{H}'\bm{x}=0, \text{ i.e. } (E_1,\dots,E_r)\bm{X}\trsp{\bm{H}'}=0.
\end{align*}
This implies that the matrix $\bm{X}\trsp{\bm{H}'}$ is not full rank, and
that all its maximal minors are equal to zero. By using the Cauchy-Binet formula that expresses the determinant of the product of two matrices 
$A\in\mathbb K^{r\times n}$ and $B\in\mathbb K^{n\times r}$ as
\begin{equation}
\label{eq:Cauchy-Binet}
\textstyle{\minor{AB}{}=\sum_{T\subset\{1..n\}, \#T=r} \minor{A}{\any,T}\minor{B}{T,\any}},
\end{equation}
each of these maximal minors can be expressed as a linear combination
of the maximal minors of the matrix $\bm{X}$. Using these minors as new
variables, we obtain a system of $\binom{n-k-1}{r}$ linear equations
in $\binom{n}{r}$ variables with coefficients over $\Fqm$, that can be
unfolded over $\Fq$ as $m\binom{n-k-1}{r}$ equations in the same
number of variables (that are searched over $\Fq$).

It is possible to solve the Rank-SD problem with the MaxMinors modeling as soon as
\begin{align}\label{eq:MM}
  \begin{cases}
    m\binom{n-k-1}{r} \ge \binom{n}{r}-1, & \text{ if the system has 1 solution},\\
    m\binom{n-k-1}{r} \ge \binom{n}{r}, & \text{ if the system has no solution}.\\
  \end{cases}
\end{align}
It is possible to improve slightly the solving by puncturing the code on $p$ positions, as long as
\begin{align}
  m\binom{n-p-k-1}{r} \ge \binom{n-p}{r}-1.
\end{align}
With the largest such $p$, the linear system has almost the same number of equations than variables. If \eqref{eq:MM} is not satisfied, then we use the hybrid approach and specialize  $a\in\{0..k\}$ columns of $\bm{X}$. The final complexity of the MaxMinors attack is bounded by
\begin{align}
  O\left(q^{ar}\binom{n-a-p}{r}^\omega\right)
\end{align}
as $n\to\infty$, where $\omega$ is the  linear algebra constant. In all our estimates, we use conservatively $\omega=2$, see Table~\ref{tab:algebraic_attacks}.

\begin{table}
  \centering
  \begin{tabular}{*{6}{|c}||c|*{3}{|c}|*{4}{|c}|}
    \hline
    $\lambda$&$q$&$m$&$n$&$k$&$r$&combi&$a$&$p$&$\mathbb C_{MM}$ & $b$ & $a$ & $p$ & $\mathbb C_{SM+}$\\\hline
    128&2&31&29&14&10&161.8&12&1&{\bf 146.1}&1 & 14 & 0 & 149.9\\\hline
    192&2&37&38&16&14&{\bf 227.4}&14&2&233.0& 1 & 13 & 0 & 230.8\\\hline
     256&2&43&44&23&13&{\bf 295.7}&20&1&300.3& 1 & 23 & 0 & 309.9\\\hline
  \end{tabular}
  \caption{Complexity of the algebraic attacks for the proposed parameters. $a$ is the hybrid parameter, $p$ the number of columns on which the code is punctured. The complexities are given in $\log_2$ bit operations. We use $\omega=2$.}
  \label{tab:algebraic_attacks}
\end{table}


We observe in Figures~\ref{fig:MMvsCombi1}, \ref{fig:MMvsCombi2}, \ref{fig:MMvsCombi3} that this approach is efficient for small $r$'s, and becomes equivalent or worse than the combinatorial approach for $r$ around the Gibert-Varshamov bound, as in this case $a$ is close to $k$ (see Figure~\ref{fig:aforMM}).
\input{figure_MM_data}

\paragraph{The Support Minors modeling}
The previous modeling is a linearization technique, that only works with a large hybrid parameter $a$ for large $r$. An altenative method is to rely on the Support Minors modeling, which was initially introduced in~\cite{BBCGPSTV20} to solve generic MinRank instances, and that uses a new set of variables. It has been adapted to instances coming from $\Fqm$-linear codes in~\cite{BBBGT22}.

%\mb{Here the vectors are row vectors...}
Write the received vector $\bm{v} = -\bm{m}\bm{G} + \bm{x}$ with $-\bm{m}\bm{G}\in C$ a codeword, and $\rank(\bm{x})= r$. Then,  $\bm{x}=\bm{v}+\bm{m}\bm{G} = (E_1,\dots,E_r)\bm{C}$  so that any row $\bm{r}_i$ of $\bm{M}(\bm{v}+\bm{m}\bm{G})\in\Fq^{m\times n}$ is in the row space of $\bm{C}$. Therefore, all the maximal minors of the matrix $\binom{\bm{r}_i}{\bm{C}}$ are equal to 0. This system is described and analyzed in~\cite{BBBGT22}, where it is shown that it contains the previous equations from the MaxMinors modeling. 

It is conjectured in~\cite{BBBGT22}, based on a careful theoretical analysis of
the system and some experimental heuristics, that it is possible to solve
this bilinear system by linear algebra on a matrix with $N$ rows
and $M$ columns, as soon as $N\ge M-1$, with:
\begin{align}
  N &=  \sum_{i = 1}^{k} \binom{n-i}{ r}\binom{k+b-1-i}{b-1} 
      - \binom{n-k-1}{ r}\binom{k+b-1}{b} \\
  &~ -  (m-1)\sum_{i=1}^{b} (-1)^{i+1} 
    \binom{k+b-i-1}{b-i}\binom{n-k-1}{r+i}.\\
  M &= \binom{k+b-1}{b}\left(\binom{n}{r} - m\binom{n-k-1}{r} \right).
\end{align}
  In this case, the final cost in $\Fq$ operations is given by
  \begin{align*}
    \mathcal{O}\left( m^2N {M }^{\omega-1}\right),
  \end{align*}
  where $\omega$ is the linear algebra constant and where the $m^2$ factor comes from expressing each $\Fqm$ operation involved in terms of $\Fq$ operations. As previously, it is possible to use an hybrid approach to reach the constraint $N\ge M-1$, or to puncture the code to get $N$ and $M$ of the same value.
The complexity estimates for the parameters sets are ploted in Figures~\ref{fig:MMvsCombi1}, \ref{fig:MMvsCombi2}, \ref{fig:MMvsCombi3}. We can see that for $q=2$, the MaxMinors modeling is (almost) always better than the Support Minors one.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-hvzk_thr.tex <==
\begin{figure}[h!]
    \pcb[codesize=\scriptsize, minlineheight=0.75\baselineskip, mode=text, width=0.98\textwidth] { 
   \textbf{Public data} : An instance of a Rank-SD problem : $\bm{H} = (I ~ \bm{H}') \in \Fqm^{\nmktn}$ and $\bm{y}\in \Fqm^{\nmk}$\\
   [\baselineskip]
   %
  \textbf{Step 1: Sample challenges} \\
  1. The prover begin to sample challenges :\\
  \pcind \pcind - Sample the first challenge : $\ch_1=\big( (\gamma_j)_{j \in \oneto{n}}, \epsilon \big)\sampler \Fqme^n \times \Fqme$ \\
  \pcind \pcind - Sample the second challenge : $\ch_2= I \subset \oneto{N} $ of parties such that $ |I| = \ell $ \\
  [\baselineskip]
  %
  \textbf{Step 2: Compute shares and their commitments} \\
  2. The prover builds a set of shares into a $(\ell+1,N)$-threshold LSSS of a random $\bm{x'}_B\in\Fqm^{n-k}$, a vector $\bm{\beta'}\in\Fqm^r$ which represents a random linearized polynomial and a random vector $\bm{a'}\in\Fqme$.\\
  3. The prover follows the protocol to build auxiliary values. For each party $i$ in a subset $S$ :\\
  \pcind \pcind - Compute $\share{\bm{x'}_B}_i = \bm{y} - \bm{H}' \share{\bm{x'}_A}_i$ and $\share{\bm{x}}_i = (\share{\bm{x}_A}_i \,||\, \share{\bm{x}_B}_i)$ \\
  \pcind \pcind - Compute $\share{z'}_i = - \sum\nolimits_{j = 1}^{n} \gamma_j \left(\share{x'_j}_i^{q^r}-\share{x'_j}_i\right)$ \\
  \pcind \pcind -  For all $k \in [1, r - 1]$ : compute $\share{w'_k}_i = \sum\nolimits_{j = 1}^{n} \gamma_j\left( \share{x'_j}_i^{q^k}-\share{x'_j}_i\right)$ \\
 \pcind \pcind - Compute $\share{\boldsymbol{\alpha'}}_i = \epsilon \cdot \share{\bm{w'}}_i + \share{\bm{a'}}_i$ and reveals $\boldsymbol{\alpha'}$\\
 4. The prover chooses $c'$ such that the protocol accepts :\\
 \pcind \pcind - Compute $c'=\epsilon z' -\dotp{\boldsymbol{\alpha'}, \bm{\beta'}}$ and builds a set of shares \\
 \pcind \pcind - Compute $\share{v'}_i = \epsilon \cdot \share{z'}_i - \dotp{\boldsymbol{\alpha'}, \share{\bm{\beta'}}_i} - \share{c'}_i$ \\
 5. The prover commits the values : \\
 \pcind \pcind - Compute for each $i\in\oneto{N}$ :  $\state_i=(\share{\bm{x'}_B}_i,\share{\bm{\beta'}}_i,\share{\bm{a'}}_i\share{c'}_i)$ and $\cmt_i=\commit{\state_i,\rho_i}$\\
 \pcind \pcind - Compute the Merkle tree root : $h_0 = \textsf{Merkle}(\cmt_1, \cdots, \cmt_N)$\\
 \pcind \pcind - Compute $h_1=\hash \left((\share{\boldsymbol{\alpha'}}_i,\share{v'}_i)_{i\in S}\right)$ \\ [\baselineskip]
 %
  \textbf{Step 3 : Output transcript} \\
  6. The prover outputs the transcript $(h_0,\ch_1,\rsp_1,\ch_2,\rsp_2)$, where $\rsp_1=h_1$ and $rsp_2=((\cmt_i)_{i\in I},\textsf{path})$, where $\textsf{path}$ is the authentication path to these commitments in the Merkle tree.
}
\vspace{-\baselineskip}
\captionof{figure}{\footnotesize{HVZK simulator for zero-knowledge proof with threshold}}
\label{hvzk_thr}
\end{figure}


==> fig-mmc.tex <==
\begin{figure}[h!]
    \pcb[codesize=\scriptsize, minlineheight=0.75\baselineskip, mode=text, width=0.98\textwidth] { 
\textbf{Inputs}\\
- Each party takes a share of the following inputs : $[\![\bm{X}]\!]\in \mathbb{F}_q^{m\times p}$, $[\![\bm{Y}]\!]\in \mathbb{F}_q^{p\times n}$ and $[\![\bm{Z}]\!]\in \mathbb{F}_q^{m\times n}$. It also need the shares $[\![\bm{A}]\!]$ of a matrix uniformly sampled from $\mathbb{F}_q^{p\times\eta}$, and $[\![\bm{C}]\!]\in \mathbb{F}_q^{m\times\eta}$ such that $\bm{C}=\bm{X}\bm{A}$.\\
1. The parties sample : $\bm{\Sigma}\leftarrow\mathbb{F}_q^{n\times\eta}$ \\
2. The parties locally computes $[\![\bm{D}]\!]=[\![\bm{Y}]\!]\bm{\Sigma} + [\![\bm{A}]\!]$ and open the shares to get $\bm{D}\in\mathbb{F}_q^{p\times\eta}$ \\
3. The parties locally computes $[\![\bm{V}]\!]=[\![\bm{X}]\!]\bm{D}-[\![\bm{C}]\!]-[\![\bm{Z}]\!]\Sigma$ and open the shares to get $\bm{V}$ \\
4. The parties outputs ACCEPT if $\bm{V}=\bm{0}$, REJECT otherwise. \\
}
\vspace{-\baselineskip}
\captionof{figure}{\footnotesize{Protocol $\Pi_{MMC}^{\eta}$}}
\end{figure}

==> fig-mpc_rsd_thr.tex <==
\begin{figure}[h!]
    \pcb[codesize=\scriptsize, minlineheight=0.75\baselineskip, mode=text, width=0.98\textwidth] { 
  \textbf{Public values.} instances of a Rank-SD problem : $\bm{H} = (I ~ \bm{H}') \in \Fqm^{\nmktn}$ and $\bm{y}\in \Fqm^{\nmk}$\\
  \textbf{Inputs.} Each party takes a share of $\share{\bm{x}_B}$ where $\bm{x}\in\Fqmn$. Let $U$ a $\Fq$-linear subspace of $\Fqm$ of dimension $r$ which contains $x_1,\dots,x_n$ and has for annihilator polynomial $L=\prod_{u\in U}(X-u)$. Each party takes a share of the following sharings as inputs : $\share{L}=X^{q^r}+\sum_{i=0}^{r-1}\share{\beta_i}X^{q^i}$, $\share{\bm{a}}$ where $\bm{a}$ is uniformly sampled from $\Fqme^r$ and $\share{c}$ such that $c=-\langle\bm{\bm{\beta}},\bm{a}\rangle$.\\[\baselineskip]
  %
  \textbf{MPC Protocol :}\\[\baselineskip]
  1. The parties sample uniformly random : $(\gamma_1,...,\gamma_n,\varepsilon)\sampler\Fqme^{n+1}$.\\
  2. The parties locally compute $\share{\bm{x}_A}=\bm{y}-\bm{H}'\share{\bm{x}_B}$ and $\share{\bm{x}} = (\share{\bm{x}_A} \,||\, \share{\bm{x}_B})$.\\
  3. The parties locally compute $\share{z} = -\sum_{j=1}^n\gamma_j(\share{x_j}^{q^r}-\share{x_j})$.\\
  4. The parties locally compute for all $k$ from 1 to $r-1$ : $\share{\omega_k} = \sum_{j=1}^n\gamma_j(\share{x_j}^{q^k}\share{x_j})$.\\
  5. The parties locally compute $\share{\bm{\alpha}}=\varepsilon\cdot \share{\bm{\omega}} + \share{\bm{a}}$.\\
  6. The parties open $\bm{\alpha}$.\\
  7. The parties locally compute $\share{v} = \varepsilon\cdot \share{z} - \langle\bm{\alpha},\share{\bm{\beta}}\rangle-\share{c}$.\\
  8. The parties open $v$.\\
  9. The parties output ACCEPT if $v=0$, and reject otherwise. 
  }
\vspace{-\baselineskip}
\captionof{figure}{\footnotesize{Protocol $\Pi^\eta$ : checking that an input is solution of an instance of Rank-SD problem}}
\label{mpc_rsd}
\end{figure}


==> figure_MM_data.tex <==
% a for MaxMinors
\pgfplotstableread{
  x      y        label
1 0 un
 2 0 un 
 3 0 un
 4 0 un 
 5 4 un
 6 7 un
 7 9 un
 8 10 un
 9 11 un
 10 12 un
 10 12 param
 11 13 un
 1 0 deux
 2 0 deux
 3 0 deux
 4 0 deux
 5 0 deux
 6 2 deux
 7 5 deux
 8 8 deux
 9 9 deux
 10 11 deux
 11 11 deux
 12 12 deux
 13 13 deux
 14 14 deux
 14 14 param
 15 14 deux
 1 0 trois
 2 0 trois
 3 0 trois
 4 0 trois
 5 4 trois
 6 9 trois
 7 13 trois
 8 15 trois
 9 16 trois
 10 18 trois
 11 19 trois
 12 19 trois
 13 20 trois
 13 20 param
 14 21 trois
}\dataFigMM


\begin{figure}[t!]
  \centering
  \begin{tikzpicture}
    \begin{axis}
      [
      legend entries={$\lambda=128$, $\lambda=192$, $\lambda=256$},
      legend pos=south east,
      height=7.0cm,
      width=12.0cm,
      xmin=0, ymin=0,
      xlabel={Target rank $r$},
      ylabel={Value of $a$},
      ]
      \addplot [
      scatter,
      only marks,
      point meta=explicit symbolic,
      scatter/classes={
        un={mark=diamond*,blue},
        deux={mark=triangle*,green},
        trois={mark=+,red},
        param={mark=*,black}    % <-- don’t add comma
      },
      ] table [meta=label] {\dataFigMM };
      \addplot [mark=none, blue] coordinates {(0,14) (11,14)};% lambda=128, k=14, rgv=11
      \addplot [mark=none, green] coordinates {(0,16) (15,16)};% lambda=128, k=16, rgv=15
      \addplot [mark=none, red]  coordinates {(0,23) (14,23)};% lambda=128, k=23, rgv=14
    \end{axis}
  \end{tikzpicture}
  \caption{Values of $a$ for the MaxMinors modeling, in terms of $r\in\{0..r_{GV}\}$ below the Gibert-Varshamov bound. The values are given for the three proposed parameter sets $(\lambda,m,n,k,r)$ equal to $(128,31,29,14,10), (192,37,38,16,14), (256,43,44,23,13)$ with $q=2$. The horizontal lines represent the value of $k$. The black points correspond to the selected value of $r$ for the proposed parameters. }
  \label{fig:aforMM}
\end{figure}


\pgfplotstableread{
  x      y        label
1 9.0 unMM
1  17.72 unC
2 15.0 unMM
2  33.72 unC
3 22.3 unMM
3  49.72 unC
4 28.8 unMM
4 65.72 unC
5 51.6 unMM
5 57.0 unSM
5 81.72 unC
6 74.7 unMM
6 78.6 unSM
6  97.72 unC
7 94.3 unMM
7 98.2 unSM
7  113.72 unC
8 112.7 unMM
8 142.6 unSM
8 129.72 unC
9 130.5 unMM
9  145.72 unC
10 146.1 unMM
10  161.72 unC
11 160.0 unMM
11 164.2 unSM
11  177.72 unC
12 178.3 unMM
12  193.72 unC
}\dataFigCombiUn

\pgfplotstableread{
  x      y        label
1 9.4 deuxMM
1  19.34 deuxC
2 15.5 deuxMM
2  35.34 deuxC
3 22.9 deuxMM
3  51.34 deuxC
4 30.1 deuxMM
4  67.34 deuxC
5 37.2 deuxMM
5  83.34 deuxC
6 53.8 deuxMM
6 60.9 deuxSM
6  99.34 deuxC
7 79.1 deuxMM
7 95.6 deuxSM
7  115.34 deuxC
8 108.2 deuxMM
8 110.8 deuxSM
8  131.34 deuxC
9 127.6 deuxMM
9 158.3 deuxSM
9  147.34 deuxC
10 153.3 deuxMM
10 151.7 deuxSM
10  163.34 deuxC
11 168.3 deuxMM
11  179.34 deuxC
12 190.6 deuxMM
12  195.34 deuxC
13 211.7 deuxMM
13  211.34 deuxC
14 233.0 deuxMM
14 230.8 deuxSM
14  227.34 deuxC
15 248.0 deuxMM
15  243.34 deuxC
16 263.0 deuxMM
16  259.34 deuxC
}\dataFigCombiDeux

\pgfplotstableread{
  x      y        label
1 10.1 troisMM
1  19.64 troisC
2 17.4 troisMM
2  42.64 troisC
3 25.5 troisMM
3  65.64 troisC
4 33.3 troisMM
4  88.64 troisC
5 58.7 troisMM
5 67.8 troisSM
5  111.64 troisC
6 95.3 troisMM
6 102.9 troisSM
6  134.64 troisC
7 133.0 troisMM
7 135.3 troisSM
7  157.64 troisC
8 163.2 troisMM
8 167.2 troisSM
8  180.64 troisC
9 241.4 troisMM
9 217.9 troisSM
9  203.64 troisC
10 223.6 troisMM
10 224.5 troisSM
10  226.64 troisC
11 249.8 troisMM
11 251.7 troisSM
11  249.64 troisC
12 272.7 troisMM
12  272.64 troisC
13 300.3 troisMM
13  295.64 troisC
14 327.8 troisMM
14  318.64 troisC
15 353.2 troisMM
15  341.64 troisC
}\dataFigCombiTrois



\begin{figure}[t!]
  \centering
  \begin{tikzpicture}
    \begin{axis}
      [
      legend entries={MM, SM, Combi},
      legend pos=south east,
      height=7.0cm,
      width=12.0cm,
      xmin=0, ymin=0,
      xlabel={Target rank $r$},
      ylabel={Value of the complexity},
      ]
      \addplot [
      scatter,
      only marks,
      point meta=explicit symbolic,
      scatter/classes={
        unMM={mark=diamond*,blue},
        unSM={mark=diamond*,green},
        unC={mark=diamond*,red}
      },
      ] table [meta=label] {\dataFigCombiUn };
    \end{axis}
  \end{tikzpicture}  
  \caption{Comparison of the MaxMinors complexity and the combinatorial attacks for the  parameters $\lambda=128$, $(2,31,29,14)$ and $r\in\{1..12\}$. Only the values of the complexities with $a<k$ are ploted.}
  \label{fig:MMvsCombi1}
\end{figure}

\begin{figure}[t!]
  \centering
  \begin{tikzpicture}
    \begin{axis}
      [
      legend entries={MM, SM, Combi},
      legend pos=south east,
      height=7.0cm,
      width=12.0cm,
      xmin=0, ymin=0,
      xlabel={Target rank $r$},
      ylabel={Value of the complexity},
      ]
      \addplot [
      scatter,
      only marks,
      point meta=explicit symbolic,
      scatter/classes={
        deuxMM={mark=diamond*,blue},
        deuxSM={mark=diamond*,green},
        deuxC={mark=diamond*,red}
      },
      ] table [meta=label] {\dataFigCombiDeux };
    \end{axis}
  \end{tikzpicture}  
  \caption{Comparison of the MaxMinors complexity and the combinatorial attacks for the  parameters $\lambda=192$, $(2,37,38,16)$ and $r\in\{1..16\}$. Only the values of the complexities with $a<k$ are ploted.}
  \label{fig:MMvsCombi2}
\end{figure}



\begin{figure}[t!]
  \centering
  \begin{tikzpicture}
    \begin{axis}
      [
      legend entries={MM, SM, Combi},
      legend pos=south east,
      height=7.0cm,
      width=12.0cm,
      xmin=0, ymin=0,
      xlabel={Target rank $r$},
      ylabel={Value of the complexity},
      ]
      \addplot [
      scatter,
      only marks,
      point meta=explicit symbolic,
      scatter/classes={
        troisMM={mark=diamond*,blue},
        troisSM={mark=diamond*,green},
        troisC={mark=diamond*,red}
      },
      ] table [meta=label] {\dataFigCombiTrois };
    \end{axis}
  \end{tikzpicture}  
  \caption{Comparison of the MaxMinors complexity and the combinatorial attacks for the  parameters $\lambda=256$, $(2,43,44,23)$ and $r\in\{1..15\}$. Only the values of the complexities with $a<k$ are ploted.}
  \label{fig:MMvsCombi3}
\end{figure}


==> forking.tex <==
\begin{lemma}{Forking lemma for 5-pass protocols}
    Let $S$ be a 5-pass signature scheme with a security parameter $k$. Let $\mathcal{A}$ be a PPT algorithm given only the public data as input. Assume that $\mathcal{A}$, after queering the random algorithms $\mathcal{O}_1$ and $\mathcal{O}_2$ polynomially often in $k$, outputs a valid signature $(\sigma_0,\sigma_1,\sigma_2,h_1,h_2)$ for a message $m$ with a non-negligeable probability. Let consider a replay of this machine $\mathcal{A}$ with the same random tape (as a Turing machine), the same response to the query corresponding to $\mathcal{O}_1$ but a different output with $\mathcal{O}_2$. Then running $\mathcal{A}$ and its reply results in two valid signatures $(\sigma_0,\sigma_1,\sigma_2,h_1,h_2)$ and $(\sigma_0,\sigma_1,\sigma'_2,h_1,h'_2)$ for the same message $m$ and $h_2\neq h'_2$ with a non negligible probability.
\end{lemma}
